Les Houches Lecture Notes on Tensor Networks

Tensor networks provide a powerful new framework for classifying and simulating correlated and topological phases of quantum matter. Their central premise is that strongly correlated matter can only be understood by studying the underlying entanglement structure and its associated (generalised) symmetries. In essence, tensor networks provide a compressed, holographic description of the complicated vacuum fluctuations in strongly correlated systems, and as such they break down the infamous many-body exponential wall. These lecture notes provide a concise overview of the most important conceptual, computational and mathematical aspects of this theory.

==> figs/MPOGroupRegular.tex <==
\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}]
	\def\l{.8};
    \def\h{.8};

	\draw[obj2, dotted] (-\l,0) -- (5*\l,0);
	
	\foreach \x in {0,1,2}{
		\draw[obj1] (2*\x*\l,2/3*\h) -- (2*\x*\l,-2/3*\h);
		\node[draw=black, line width=.7pt, fill=gray!20, rectangle, inner sep=2pt, rounded corners=2pt] at (2*\x*\l,0) {$\sss g$};
	}
\end{tikzpicture}

==> figs/MPOSingle.tex <==
\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}]
	\def\l{.8};
    \def\h{.8};

	\draw[obj2] (-2/3*\l,0) -- (2/3*\l,0);
    \draw[obj1] (0,2/3*\h) -- (0,-2/3*\h);
    \node[draw=black, line width=.7pt, fill=gray!20, rectangle, inner sep=3.8pt, rounded corners=2pt] at (0,0) {};
    \node[anchor=south] at (-\l/3,0) {$\sss a$};
\end{tikzpicture}
